Protocol Dialects as Formal Patterns: A Composable Theory of Lingos -- Technical report

Protocol dialects are methods for modifying protocols that provide light-weight security, especially against easy attacks that can lead to more serious ones. A lingo is a dialect's key security component by making attackers unable to "speak" the lingo. A lingo's "talk" changes all the time, becoming a moving target for attackers. We present several kinds of lingo transformations and compositions to generate stronger lingos from simpler ones, thus making dialects more secure.

==> text/cathy.tex <==
This section consists of material that is probably going to go into different sections.
\subsection{Protocol Dialect Desiderata}
In this section we set forth some properties of protocol dialects. We note that these properties are not always completely compatible, and it may be necessary to trade off different properties against each other.
\begin{itemize}
    \item Dialects should provide a minimal computational burden
    \item The decisions that need to made when configuring a dialect should be minimal.  Misconfiguration is one of the major causes of security vulnerabilities.
    \item In order to minimize decisions, dialects need to be as protocol-independent as possible.
    \item In some cases, avoiding regulatory restrictions, e.g. export controls, may be desirable in order
	to avoid paperwork overhead. If so, this
	may affect the strength of the algorithms we choose, and what we use the algorithms for.  E.g. we 	may want to avoid anything that looks like encryption.
    \item Dialects should be easy to implement, in order to avoid implementation mistakes.
    \item If a dialect is running over a lower-level protocol, it should not try to replicate the lower-level protocol's work.  However, it should do as much as possible not to interfere with the lower-level protocol doing its job.
\end{itemize}
\subsection{Lingo Properties}
In this section we give a definition of the properties that lingos need to have in order to provide protection against different types of attackers. We first give a definition of security that applies to a large number of attack scenarios, in particular those that occur when we attempt to reuse lingos with the same parameters.

\begin{definition}
Let $f,g$ be a lingo, and let $p$ be a set of parameters.   We define $f_p$ and $g_p$ be the functions $f$ and $g$ with the parameters fixed at $p$. 
\end{definition}

\begin{definition}
Let $n$ be a natural number . We say that a function pair $f,g$ is $n$-\emph{unspoofable} if, after seeing $n$ examples $f_p(m_1), \ldots, f_p(m_n)$, the attacker can  produce $f_p(m')$ for some $m'$ chosen by the attacker with negligible probability.  We say that $f,g$ is $n$-\emph{unmatchable} if it is $n$-uspoofable, and, if $n >0$, then given $f_p(m)$ and a sequence  $f_p'(m_1), \ldots. f_p'(m_n)$, the probability of the attacker's guessing whether or not $p = p'$ is negligibly greater than chance.

\end{definition}

In our automated analysis we will, as is the case with other symbolic analysis techniques, interpret "negligible" as "zero" probability.

The definition of unspoofability captures the fact that an attacker can not only spoof a message by finding the transformation $f_p$ and applying it to a different message, but by making direct alterations in $f_p(m)$ that result in a new message $f_p(m')$.  Thus, for example, supppose that $f_p(m) = r \oplus m$, where $r$ is a random number, and the attacker knows that if $m$ is a legal message, then so is the result of flipping the second bit of $m$ to obtain $m'$.   Then $010^{k-2} \oplus r \oplus m = oplus r \oplus m'$.

The definition of unmatchability  applies to the case in which an attacker wants to pass off an old message $f\_p(m)$ as a current one.  The only way that this can happen is if either 1) The combination of $f, g$, and $p$ is applied at most $n +1$ times, and 2) $f, g$ is $n$-unmatchable.  Note that any zero-unspoofable function is trivially zero-unmatchable.



We now show how these definitions apply to different attacker models.

\begin{enumerate}
    \item \emph{Off-Path Attacker}  The off-path attackers sees no messages that are not intended for it.  Thus, since it is not part of the enclave, it sees no dialected messages at all.   Thus, assuming the the dialect and parameters are not subject to being leaked by some other means, it is enough to use a single zero-unspoofable function, and to never change the parameters at all.  
    \item \emph{On-path Attacker, parameters change each time}  In this case the attacker can read messages and send messages as other principals, but can not intercept messages or alter them in flight.   In this case a  zero-unspoofable function pair $f,g$ can be used. 
    \item \emph{On-path Attacker, parameters change at after $k$ units of time have passed}  In this case we would want to pick an $n$-unspoofable function such that it is extremely unlikely that  more than $n$ messages will be sent during $k$ time units. In general, you would want to use this if $n$ would have to be relatively large. 
    \item \emph{On-path Attacker, parameters change  after $n$ messages have been sent}  In this case we would want to pick an $n$-unspoofable or $n$-unmatchable function. This would work best if $n$ is relatively small.
\end{enumerate}








==> text/dialects-as-moving-targets.tex <==
Every dialect should be a moving target, but some dialects move faster than others. We present a new dialect that changes its behavior and transformations over time, introducing a new layer of enhanced obfuscation and unpredictability. Remember that a dialect has the same lingo at all times (i.e., the lingo received as a parameter of the dialect). It is still a moving target, because the \emph{parameters} of the fixed lingo are always changing. Faster moving targets can be achieved through what we call \emph{dynamic} dialects, where the current lingo changes dynamically. This frequent change of the communication format imposes a serious burden on intruders, because even if a specific lingo is successfully broken, the dialect will change this lingo after some time, forcing the intruder to start all over again its malicious efforts. We propose two approaches: aperiodic and periodic. \victor{Remember to update the following accordingly to Security Section} As detailed further in Section \ref{sec:security}, one can obtain desirable security outcomes when lingos change faster than the time an intruder takes in correctly guessing and reverting each lingo transformation.

\begin{definition}[Dynamic Dialect]
A dynamic dialect $\dlct$ is a dialect of the form
$\dlct_{\vec{\Lambda}}(\proto)$, where $\vec{\Lambda}$ is a vector of lingos and $\proto$ is the underlying protocol. It must be noted that all lingos in $\vec{\Lambda}$ must be over the same data type, that is $\vec{\Lambda} = [\Lambda_1(D),...,\Lambda_n(D)]$ for a vector of $n$ lingos. Moreover, as with static dialects, the protocol $\proto$ must be over that same data type $D$. Dynamic dialects introduce a new attribute, \texttt{current-lingo}, and a new function, \texttt{choice}. The \texttt{current-lingo} attribute serves as a flag to know which is the current lingo for the dialect to apply. The \texttt{choice} function takes care of updating the current lingo by throwing a dice, in a similar way as it is done in horizontal compositions. The \texttt{choice} function is defined as $\texttt{choice} : N \rightarrow Qid$.
The transformation adds a new actor subclass of the form
``$    \texttt{class}\ \textit{DynamicDialect} \mid \texttt{current-lingo} : CL$"
with
``$    \texttt{subclass}\ \textit{DynamicDialect} < \textit{Dialect}
$".
\end{definition}

\subsection{Aperiodic Dialects}\label{subsec:aperiodic-dialects}

Dialects are moving targets because the parameter, used to obfuscate and de-obfuscate, changes per message. Dialects can move faster by changing the lingo they use to communicate with their peers through Dynamic Dialects in many different ways. Aperiodic Dialects is one of our two approaches. The main idea of aperiodic dialects is to change the current lingo after a certain bound on the number of sent messages has been reached. This number is tied to the peer, so different peers will change lingo at different 'times', adding extra entropy. Let us describe aperiodic dialects through an example. Figure~\ref{fig:aperiodic-dialect} shows a snapshot of a network between client and server. Both actors use an aperiodic dynamic dialect to obfuscate the communication. Let the vector of Lingos $\vec{\Lambda} = \{XOR,D\&C\}$. The communication in the snapshot can be divided into two phases, each of them applying one lingo. The length of each phase is $MB \in \mathbb{N}$, as set by the aperiodic dialect. Once the number of messages exchanged between client and server reaches the message bound $MB$, the dialect chooses a new lingo. During the first phase, $XOR$ is applied. During the second phase, $D\&C$ is chosen and used to obfuscate the communication. Notice that in both phases the communication is obfuscated with a different parameter per message. 
%The former uses a message bound to change the current lingo in a communication between two principals. The later, which is fully explained in Section \ref{subsec:periodic-dialects}, uses a time bound to change the current lingo used in a Dialect for all communications.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/aperiodic-dialect.pdf}
\caption{Sequence of messages between server and client using aperiodic dialect meta-objects.}
\label{fig:aperiodic-dialect}
\end{figure}


\begin{definition}[Aperiodic dialect]
    Given a dynamic dialect $\dlct_{\vec{\Lambda}}(\proto)$ and a message bound $\mu \in \mathbb{N}$, an aperiodic dialect $\dlct_{\vec{\Lambda}}^{\mu}(\proto)$ defines a new actor subclass of the form
``$    \texttt{class}\ \textit{AperiodicDialect} \mid \texttt{msg-bound} : \mu, \texttt{cl-peer} : Map\{Oid, Triplet\{Nat, Qid, Nat\}\}$"
with
``$    \texttt{subclass}\ \textit{AperiodicDialect} < \textit{DynamicDialect}
$".
The {\texttt{msg-bound}} attribute contains the number of messages the dialect will transform with some lingo before changing phase. The \texttt{cl-peer} attribute is a map from object identifiers to triplets. The first element of the triplet is a natural number representing the current number of messages exchanged with the entry peer. The second element is a quoted identifier for the lingo to be used with the peer. The third element is the number of times the lingo has changed, and is used in the computation of the next lingo for that peer.
\end{definition}

\begin{example}[Aperiodic Dialect over MQTT]
    \victor{Use the example that uses XOR and D\&C over MQTT}
\end{example}

\subsection{Periodic Dialects}\label{subsec:periodic-dialects}

Periodic dialects are a specialization of dynamic dialects that change lingos periodically through time. Periodic dialects are our contribution as another case of dynamic Dialects, a new idea in the field of Dialects.

\begin{definition}[Periodic dialect]
    Given a dynamic dialect $\dlct_{\vec{\Lambda}}(\proto)$ and a period $\tau \in \mathbb{N}$, a periodic dialect $\dlct_{\vec{\Lambda}}^{\tau}(\proto)$ defines a new actor subclass of the form
``$    \texttt{class}\ \textit{PeriodicDialect} \mid \texttt{period} : \tau, \texttt{p-counter} : PC, \texttt{p-number} : PN, \texttt{prior-lingo} : PL$"
with
``$    \texttt{subclass}\ \textit{PeriodicDialect} < \textit{DynamicDialect}
$".
The {\texttt{period}} attribute contains the length of the period. \texttt{p-counter} stores how much time is left for the current period. \texttt{p-number} has the number of times we have changed periods. The \texttt{prior-lingo} attribute stores the previous period's current-lingo value. In this way, up to some clock skew $\tau_{skew}$ there are two lingos that can be applied in case a delayed message from the previous period arrives in the next $\tau_{skew}$ times into the next period.
\end{definition}

A periodic dialect is responsible for defining how time passing affects him. For that purpose, we have the two equations of Figure \ref{fig:eq-delta-periodic}, defining the delta function over periodic dialects. The first function captures the case where the time advancement falls into the same period, in which case the period counter is decreased. The second equation captures the other case, where the time advancement is sufficient to change to the next period. The period change is defined by setting the period at the beginning, increasing the number of periods and updating both the current lingo, with the choice function, and the prior lingo, with the current lingo value. In both cases, the time advancement is passed down the configuration of objects.

\begin{figure}
    \centering
\begin{verbatim}
*** Case limit is NOT reached
ceq delta(< O : DC:PeriodicDialect{DL,P} | p-counter : T, 
                                           conf : Cfg, 
                                           Atts >, Ti) = 
          < O : DC:PeriodicDialect{DL,P} | p-counter : T monus Ti, 
                                           conf : delta(Cfg, Ti), 
                                           Atts >
    if T > Ti [dnt] .

*** Case limit IS reached
ceq delta(< O : DC:PeriodicDialect{DL,P} | p-counter : T, 
                                           conf : Cfg, 
                                           Atts >, Ti) = 
    delta(< O : DC:PeriodicDialect{DL,P} | p-counter : 0, 
                                           conf : delta(Cfg, Ti), 
                                           Atts >, Ti monus T)
    if T <= Ti /\ T =/= 0 [dnt] .
\end{verbatim}
    \caption{Equations modeling the semantics of time passing in Periodic Dialects.}
    \label{fig:eq-delta-periodic}
\end{figure}

We can illustrate the behavior of a periodic dialect with the example in Figure~\ref{fig:transform-vs-choice}. The vertical axis represents time advancing from top to bottom. During a {\em time phase} $TP$, all participants of a particular modified protocol use the same {\em current lingo}. At {\em phase boundaries}, the phase changes, and then dialects use their $\choice$ function to agree on a new current lingo, as depicted by the dashed horizontal line. In the figure, during the first phase {\tt XOR} is the current lingo, and {\tt D\&C} becomes the current lingo during the second phase. Note that, during each phase, the lingo parameters ($s_1,s_2,\ldots, s_n$ for {\tt XOR}, resp. $s_{n+1},s_{n+2},\ldots, s_k$ for {\tt D\&C}) change all the time in a synchronized fashion between server and client. %The reasoning behind this is that functionality provided by the \texttt{update} function continues operating the same as in a static dialect.

\begin{figure}[t] 
    \centering
\includegraphics[width=\linewidth]{figures/periodic-dialect.pdf}
\caption{Example sequence of two principals using a dynamic periodic dialect.}
\label{fig:transform-vs-choice}
\end{figure}

\begin{example}[Periodic Dialect over MQTT]
\victor{Show \texttt{per-xor-mqtt.maude} with constant and variable delays.}
\end{example}

Periodic dialects make an essential use of time. This raises a need for {\em time synchronization}. Protocol objects may run in different distributed devices, so disagreements on a common view of time could lead to divergent and incompatible lingo transformations. We assume (but leave implicit) that in a periodic dialect environment: i) all dialect meta-objects share a canonical view of time, ii) objects perform actions in lockstep by synchronizing their local clocks, and iii) periodic dialects remain synchronized during the entire duration of the communication process employing well-known time synchronization protocols, such as NTP~\cite{rfc5905} or its secure version NTS~\cite{rfc8915}. We believe these assumptions ensure that all meta-objects will change their current lingo at, approximately, the same time.

\victor{What follows can be added as an appendix.}

\paragraph{Modeling time}

To model time for periodic dialects in Maude, we have integrated into our framework a subset of Real-Time Maude \cite{olveczky2007semantics}. Recall that our model considers principals as objects (or meta-objects in the case of dialects) floating in a common environment, representing the network.
\begin{comment}
To represent time, we use parametric rewrite theories accepting a time domain as argument, introduced in the form of a new sort \texttt{Time}; %all objects in the network are endowed with local clocks of sort \texttt{Time}; and the environment is wrapped with a global clock of sort \texttt{Time}.
\end{comment}
The subset of Real-Time Maude introduces a new sort \texttt{Time} and the dialect system is wrapped within an operator of sort \texttt{ClockedSystem}. This operator, $\texttt{NET} \ in \ time \ \texttt{GC}$, encapsulates the network $\texttt{NET}$ where we have objects and meta-objects, and adds a global clock $\texttt{GC}$. To represent time, we use the domain of natural numbers $\mathbb{N}$. Real-time Maude also introduces two new functions to the equational theory: (1) a local \emph{time advancement} (\texttt{delta}) function which, given a subject (object or message) and the quantity of time to advance, mutates the subject to advance its local clocks and ensure its internal state is coherent wrt. the indicated time span; and (2) a \emph{maximum time elapse} (\texttt{mte}) function which, given a subject, yields the maximum quantity of time that may safely pass before some object must execute an action. Real-Time Maude also introduces a new class of rewrite rules: time rules. Contrary to our dialect framework rules that are instantaneous, time rules model the passage of time by adding time to the global clock of the clocked system. Figure \ref{fig:time-rules} depicts three rules: 
\begin{enumerate}
    \item Rule labelled \texttt{tick} recurrently ensures time advances for all principals in the network following a two-step process: first, (a) the \emph{maximum time elapse} is evaluated on all objects and messages of the environment to discover an appropriate amount $t$ with which to advance time before someone must perform an action, (b) the \emph{time advancement} is recursively applied to the entire environment to advance time by $t$ units, and (c) the global environment clock is also advanced $t$ units.
    \item Rule labelled \texttt{tick+1} advances time by the minimum unit of $\mathbb{N}$.
    \item Rule labelled \texttt{tick+mte} models the passage of time by function \texttt{mte}.
\end{enumerate}
Notice that the fist two rules are not executable. The reasoning behind is to make the experiments finite. \victor{We might want to expand this. Footnote?}

\begin{figure}
    \centering
\begin{verbatim}
crl [tick] :
        { C } in time T' => { delta(C, T) } in time (T' + T)
    if T <= mte(C) [nonexec] .
    
*** Rule to advance time one by one independent of mte
rl [tick+1] :
    { C } in time T => {delta(C, 1)} in time (T + 1) [nonexec] .

*** Rule to advance time by mte
crl [tick+mte] :
    ({ C } in time T) => ({delta(C, T')} in time T + T')
    if  T' := mte(C) /\
        T' >= 1 /\
        T' =/= INF .
\end{verbatim}
    \caption{Rules modelling the passage of time.}
    \label{fig:time-rules}
\end{figure}

In the case of periodic dynamic dialects, we consider the time that messages take to traverse the network as the sole source of time advancement. For this purpose, we wrap messages with a special \texttt{delay} operator which represents the time needed to traverse the network between two principals. This operator contains the message and a timer. The \emph{time advancement} is defined such that the timer counts down as time advances, and once it reaches zero, the message is unwrapped and the operator is discarded, allowing the destination object to take it from the environment normally. The definition of the \emph{maximum time elapse} function enables the framework to safely advance the simulation time without stopping until one or more \texttt{delay} operators are ready to be unwrapped. %On the other hand, we consider the local computations of principals (processing messages, applying dialects, etc.) to be considerable faster, and thus use instantaneous rules for the rest of the model.

%Further comments on delay (variable delay)
As an extra note on delays, our framework considers two kinds of delay timers: constant and variable delays. Constant delays are the simplest form of delay, making all messages in the network be sent with the same delay value. This allows us to run the non-timed models with a notion of time. Variable delays, on the other hand, give way to a more complex and flexible environment. With variable delays, each message, when sent, might have a different delay, allowing for cases where a message is received before another one that was sent earlier to the same principal.

==> text/security.tex <==
\subsection{Goals}\label{sec:security-goals}

\subsection{Attacker Model}\label{sec:attacker}

\subsection{Experiments}\label{sec:security-experiments}
We have expressed our attacker model as an specification in Maude, enabling exhaustive simulation of traces where communication has a configurable amount of influence exerted by an intruder. Using tools available in the Maude interpreter and ecosystem, such as (statistical) model checking \cite{} and \emph{narrowing} \cite{}, this enables computer-aided formal reasoning of how attacker capabilities affect the security properties of our proposed framework.

\paragraph{Attacker objects and wrappers} Recall that our framework models a communication network as a set of objects floating in a common environment, and which communicate by sending messages to each other. We model each attacker as one \emph{attacker object} and a series of attacker-controlled \emph{malicious wrappers}. An \emph{attacker object} resides in the environment like a regular principal, representing the presence of the attacker as an independent agent in the network, and its attributes privately store the attacker's local state and knowledge. Depending on the considered attacker capabilities, an attacker object may be able to communicate directly with both honest participants and other attacker objects. 

On the other hand, \emph{malicious wrappers} are special meta-objects which wrap victim objects and are remotely controlled by an \emph{attacker object}. Similarly to an spy agent deployed to foreign territory, these wrappers can perform both passive and active actions affecting the communications of the victim on behalf of their owner. In the passive case, these wrappers can eavesdrop the communications of the victim by cloning all incoming and outgoing messages and then sending a copy to their owner, which can then store such messages in their local stores for further processing. This transfer of cloned messages is not performed using regular messages, but is instead modeled as an out-of-band communication, meaning that the communication between attackers and the wrappers they control is assumed to be undetectable, unbreakable and uninterruptible. In the active case, wrappers may also selectively intercept messages to then drop or modify them, enabling the simulation of scenarios where the victim is under a successful denial of service attack, or where the local communication channels of the victim have been (partially) compromised.

Our model uses realistic network discovery rules that effectively focus on the security and effect of using dialects. Objects may not enumerate the rest of the objects of the environment, and such network discovery must be performed at the protocol level by, e.g., sending broadcast messages and then gathering replies. Consequently, attacker objects which remain passive, or are sufficiently selective with the messages they respond to, will effectively remain undetectable to other principals in the network. Similarly, victim objects are oblivious to the fact they may be wrapped by one or more malicious wrappers, and must actively work to prevent malicious influence by judiciously configuring and using dialects.

\paragraph{Attacker knowledge} Attacker knowledge is represented as local state in the corresponding \emph{attacker object} as a pair of stores $(\mathcal{R}, \mathcal{C})$, respectively called the \emph{captured message registry} and the \emph{cleartext message registry}. As attackers eavesdrop communications of their victims through their \emph{malicious wrappers}, the captured messages are locally stored in $\mathcal{R}$ as a set of records of the form $(s,d,m,t,\Gamma)$ where $m$ is the captured message, $s$ and $t$ are the source and destination objects of the message, $t$ is the timestamp of the moment when the message was captured by the proxy, and finally the \emph{hidden context data} $\Gamma$ bundles some bookkeeping information required by our model to operate. Note that the messages are stored as they are captured from the network and are thus likely to be \emph{dialected} (i.e., they may be unreadable due to the effect of dialects), but networking data such as the source and destination is not affected by dialects. 

As messages are gathered and time passes, the attacker may be able to learn enough information to reveal the captured dialected messages and enrich her local knowledge, storing the clear messages in a second registry. For this purpose, we model the following four-step process to populate the second registry $\mathcal{C}$ with cleartext messages: first, (1) a candidate dialected message is selected from the registry $\mathcal{R}$; secondly, (2) the attacker discovers information of what dialects and lingos were originally used to obfuscate the selected message, alongside the corresponding lingo parameters; then (3) the message contents are revealed by reverting the effect of dialects; and finally (4) the obtained cleartext equivalent, alongside the discovered dialect and lingo information, is stored in the registry $\mathcal{C}$. This process is regulated according to the capabilities of the attacker, in the sense that it will not be performed with messages where discovering how to revert the effect of dialects is deemed too difficult.

The \emph{cleartext message registry} $\mathcal{C}$ contains a set of records $(s,d,m,t,c,D,L,P)$, whose first components are exactly as in $\mathcal{R}$, but the last components extend those in $\mathcal{R}$ as follows: $c$ is the cleartext message (i.e., $m$ but with the effects of dialects reverted), $D$ contains information about the dialects that originally obfuscated $c$ into $m$, $L$ contains information about the lingos of $D$ that performed the corresponding transformations, and $P$ comprises the parameters that were used with the lingos in $L$. Using the information $D$, $L$ and $P$, the cleartext message $c$ can be revealed from the dialected message $m$. This information is obtained from $\mathcal{R}$, where it remains hidden in the special parameter $\Gamma$, and where it cannot be read or modified by the attacker.

\paragraph{Attacker capabilities} We consider a series of rules, called the \emph{attacker capabilities}, which describe when it is possible to reveal messages from $\mathcal{R}$ and store the new knowledge gained in $\mathcal{C}$. When a rule $r$ is evaluated, it assigns a probability $p_r$ to each message $m$, expressing how probable it is that the attacker may be able to immediately reveal the contents of the message and its associated dialect information, where a value of $0$ indicates that the message is impossible to reveal and $1$ means that revealing the message is trivial. Because the attacker only needs at least one technique to succeed to reveal a message, the probabilities of evaluating several rules are additive, i.e., when evaluating a set of rules $R$ on a message $m$, the probability of revealing $m$ is $\operatorname{min}(\sum_{r \in R} p_r, 1)$.

Even though dialects are varied, and the methods that an attacker may use to guess dialects and deobfuscate messages define a wide spectrum, we propose a particular set of abstract, \emph{parametric} rules which describe, in general terms, how an intruder may be able to successfully perform such a task without detailing particular techniques:
\begin{enumerate}
    \item \textbf{Messages older than $t_{\rm max}$:} as time advances, the attacker has more chances to successfully use her resources and exert her influence to guess the dialect and lingo information and learn how to effectively reveal messages. The argument $t_{\rm max}$ is a probability distribution describing how probable it is that a message can be revealed if its age is equal to or greater than $t_{\rm max}$ units of time\footnote{In Maude, probability distributions are modeled as total functions $f : \mathbb{N} \rightarrow \left[0,1\right] \subset \mathbb{R}$.}. For each entry $(s,d,m,t,\Gamma)$ in $\mathcal{R}$, the age of the message is defined as the difference between its timestamp $t$ and the current time $t_{\rm now}$. Thus, the probability that $m$ can be revealed is then defined as the evaluation of the probability distribution $t_{\rm max}(t_{\rm now} - t)$.
    \item \textbf{Lingo \emph{weakly} reused more than $w_{\rm max}$ times:} reusing the same lingos several times may give hints to the intruder, giving her an advantage. We say that a lingo has been \emph{weakly} reused if it has been used more than once but with different parameters each time. Let $\operatorname{count}(\delta, \mathcal{R})$ be the number of times the lingo $\delta$ has been reused (with any parameter) in messages in $\mathcal{R}$, i.e., the number of entries where the message $m$ was transformed with $\delta$. For each entry $(s,d,m,t,\Gamma)$ in $\mathcal{R}$, the framework obtains from $\Gamma$ the set of lingos $\Delta$ that were used to transform it and then it computes the maximum count of weakly reused lingos, i.e., $n_m = \operatorname{max}_{\delta \in \Delta}(\operatorname{count}(\delta, \mathcal{R}))$. This count is then used to evaluate the probability distribution, assigning $w_{\rm max}(n_m)$ to $m$.
    \item \textbf{Lingo \emph{strongly} reused more than $s_{\rm max}$ times:} similarly to weak lingo reuse, strong lingo reuse is caused when a lingo is used more than once, but with identical parameters. This form of reuse is worse from a security standpoint for many lingos. Let $\operatorname{count}(\delta, \rho, \mathcal{R})$ be the number of times the lingo $\delta$ has been reused with parameters $\rho$ in messages in $\mathcal{R}$, i.e., the number of entries where the message $m$ was transformed with lingo $\delta$ and parameters $\rho$. For each entry $(s,d,m,t,\Gamma)$ in $\mathcal{R}$, the framework obtains from $\Gamma$ the set of lingos and parameters $\Delta = \{\delta_i, \rho_i\}_i$ that were used to transform it and then it computes the maximum count of strongly reused lingos, i.e., $n_m = \operatorname{max}_{(\delta, \rho) \in \Delta}(\operatorname{count}(\delta, \rho, \mathcal{R}))$. This count is then used to evaluate the probability distribution, assigning $s_{\rm max}(n_m)$ to $m$.
    \item \textbf{Messages that are already cleartext:} if a captured message has not been dialected and looks like a valid protocol message, the attacker may vacuously reveal it immediately, i.e., if a message $m$ has not been transformed by any lingo then its probability is assigned to $1$, and $0$ otherwise. Note that in this case the resulting entry in $\mathcal{C}$ has the dialects, lingo and parameter information $D$, $L$ and $P$ set to null values, as nothing else than the message contents has been learned.
\end{enumerate}

Once each message $m$ in $\mathcal{R}$ has a probability $p$ assigned from evaluating all available rules, the system generates a (pseudo-)random real number $r$ in the interval $\left[0,1\right]$ and compares it to $p$, revealing $m$ if $r \leq p$.

The tuple of values used for the parameters of the described attacker capabilities, $(t_{\rm max}, w_{\rm max}, s_{\rm max})$, is called the \emph{attacker advantage}. Depending on the provided values, the attacker will reveal some messages faster or slower, and may be unable to reveal some messages altogether.
